Omnipredictors

Loss minimization is a dominant paradigm in machine learning, where a predictor is trained to minimize some loss function that depends on an uncertain event (e.g., "will it rain tomorrow?''). Different loss functions imply different learning algorithms and, at times, very different predictors. While widespread and appealing, a clear drawback of this approach is that the loss function may not be known at the time of learning, requiring the algorithm to use a best-guess loss function. We suggest a rigorous new paradigm for loss minimization in machine learning where the loss function can be ignored at the time of learning and only be taken into account when deciding an action. We introduce the notion of an (${\mathcal{L}},\mathcal{C}$)-omnipredictor, which could be used to optimize any loss in a family ${\mathcal{L}}$. Once the loss function is set, the outputs of the predictor can be post-processed (a simple univariate data-independent transformation of individual predictions) to do well compared with any hypothesis from the class $\mathcal{C}$. The post processing is essentially what one would perform if the outputs of the predictor were true probabilities of the uncertain events. In a sense, omnipredictors extract all the predictive power from the class $\mathcal{C}$, irrespective of the loss function in $\mathcal{L}$. We show that such "loss-oblivious'' learning is feasible through a connection to multicalibration, a notion introduced in the context of algorithmic fairness. In addition, we show how multicalibration can be viewed as a solution concept for agnostic boosting, shedding new light on past results. Finally, we transfer our insights back to the context of algorithmic fairness by providing omnipredictors for multi-group loss minimization.

==> algorithm.tex <==
\subsection{Reducing multi-calibration to weak agnostic learning} 

Informally, a weak agnostic learner is an algorithm that is able to detect non-trivial correlation between the labels and functions in a class. 
We use the definition of a weak agnostic learner for a class $\mC$ of functions following Kalai and Kanade.

\begin{definition}
    For $\alpha' \leq \alpha$, an $(\alpha, \alpha')$ weak learner for a class $\mC$ takes samples from a distribution $\D$ on $\X \times \pmo$. If there exists $c \in \mC$ such that $\E_{\D}[c(\x) \z] \geq \alpha$
    then with probability $1- \delta$ the weak learner returns a hypothesis $c' \in \mC$ such that $\E_{\D}[c'(\x) \z] \geq \alpha'$. The sample complexity and running time depend on $\alpha, \alpha'$ and $\delta$ and the dimensionality of the data. 
\end{definition}

Note that  $\alpha' \leq \alpha$, and indeed Kalai and Kanade consider $\alpha' = \gamma \alpha$ for some $\gamma < 1$. One can allow the learner to be improper, meaning that it returns $c' \in \mC'$ for some different, possibly broader class of function $\mC' \neq \mC$. Our results will apply even with these changes, but for simplicity we work with proper learners. 

One can reduce the problem of detecting if a partition is multi-calibrated to a weak agnostic learning problem. While Equation \eqref{eq:m-cal} does require finding significant correlation with $\mC$, $\y \in \zo$, $\y - p_i$ can take values outside $\zo$, whereas our definition of weak learner for $\mC$ expects $\pmo$ labels. There are a couple of ways of dealing with this issue in the literature.


\paragraph {Distribution Reweighting.}
Define the distribution $\D_i^0$ on $S_i \times \pmo$ as follows:
with probability $1/2$ we sample $\x \sim \D_i|\y =1$ and output $(\x, \z = 1)$, and with probability $1/2$ we sample $\x \sim \D_i|\y = 0$ and output $(\x, \z = -1)$. It is easy to check that this is equivalent to
\begin{align}
    \label{eq:d0}
    \D_i^0(x, 1) = \frac{\D_i(x,1)}{2p_i}, \ \D_i^0(x, -1) = \frac{\D_i(x, 0)}{2(1 - p_i)} 
\end{align} 
and that $\E_{\z \sim \D^0_i}[\z] = 0$.

\begin{lemma}
\label{lem:reweight}
$\mS$ is $\alpha$-multi-calibrated for $\mC, \D$ iff the following condition holds for all $i \in [m]$ and $c \in \mC$:
    \[ \abs{\E_{(\x, \z) \sim \D^0_i}[c(\x) \z]} \leq \alpha/2.\] 
\end{lemma}
\begin{proof}
    Let $(\x', \z) \sim \D_i^0$, and $(\x, \y) \sim \D$. Then we claim that  
    \begin{align*} 
        \E_{\D^0_i} [c(\x')\z] &= \frac{\E_{\D_i}[c(\x)(\y - p_i)]}{2p_i(1 - p_i)}.
    \end{align*}
    We can rewrite Equation \eqref{eq:d0} as
    \begin{align}
    \label{eq:d0-single}
        D_i^0(x, 2y -1) = D_i(x, y) \frac{ (1 - 2p_i)y + p_i}{2p_i(1 - p_i)}.
    \end{align} 
    Hence    
    \begin{align*}
        \E_{(\x', \z) \sim \D^0_i}[c(\x') \z] = \E_{(x, \y) \sim D_i}
        \left[\frac{ (1 - 2p_i)\y + p_i}{2p_i(1 - p_i)}c(\x)(2\y -1)\right] = \E_{(x, \y) \sim D_i}\left[c(\x)\frac{ \y - p_i}{2p_i(1 - p_i)}\right].
    \end{align*}
\end{proof}

Given random samples from $\D_i$ one can generate a random sample from $\D^0_i$ using rejection sampling, using $O(1/p_i(1 - p_i))$ samples. 



\eat{
Hence 
Rather than shifting the inputs, we reweight them to make the labels unbiased: every sample labelled $1$ is scaled by $(1 - p_i)$ and every sample labelled $0$ is scaled by $p_i$. (entirely standard, but we present it below for completeness). In this reweighted scheme, we require a weak learner to produce $c \in \mC$ that has correlation at least $\alpha$. 




\begin{lemma}
\label{def:mcab}
$D_i^0$ defined in Equation \eqref{eq:d0} is a distribution, where the labels are unbiased: $\E_{\D^0_i}[\y] = 1/2$.
The partition $\mS$ is $\alpha$-\mcbd\ for $\mC, \D$ iff for every $i \in [m]$ and $c \in \mC$, it holds that
\begin{align}
\label{eq:m-cal3}
 \abs{ \E_{(\x,\y)\sim \D_i^0} [c(\x) \y] } \leq \alpha.
\end{align}
\end{lemma}
\begin{proof}
One can verify that $\D_i^0$ is a distribution since
\[ \E_{(\x, \y) \sim \D_i} \left[\frac{\D^0_i(\x, \y)}{\D_i(\x, \y)} \right] = \fr{1 -\eta_i^2}\E_{(\x, \y) \sim \D_i} [1 - \y \eta_i] = 1, \]
and that the labels are unbiased under $\D^0_i$ since
\[ \E_{(\x, \y)\sim \D^0_i}[\y] = \E_{(\x, \y) \sim \D_i} \left[\y\frac{1 - \y  \eta_i}{1 - \eta_i^2}\right] = \fr{1 -\eta_i^2} \E_{(\x, \y) \sim \D_i} [\y -  \y^2\eta_i] = 0\]
where we use $\E_{\D_i}[\y] = \eta_i$ and $\y^2 =1$ since $\y \in \pmo$.
We have 
\begin{align*} 
    \E_{(\x,\y)\sim \D_i^0} [c(\x) \y]  &=  \E_{(\x,\y)\sim \D_i} \left[\frac{\D_i^0(\x, \y)}{\D_i(\x, \y)} c(\x) \y\right] =  \E_{(\x,\y)\sim \D_i} \left[ \frac{1 - \y \eta_i}{ 1 - \eta_i^2} c(\x) \y\right]\\
    & = \fr{1 - \eta_i^2} \E_{(\x,\y)\sim \D_i}[c(\x)(\y - \y^2\eta_i)] = \fr{1 - \eta_i^2} \E_{(\x,\y)\sim \D_i}[c(\x)(\y - \eta_i)].
\end{align*}
It follows that Equations \eqref{eq:m-cal2} and \eqref{eq:m-cal3} are equivalent.
\end{proof}

Alternately, following Kalai-Kanade and Feldman, one can probably keep the marginal distribution on $\X$ unchanged, and just add label noise. 
}



\subsection{Sample efficiency}

In practice, we are given random samples from the distribution $\D$, which means that we cannot estimate quantities like $\Var_{D_i}[\y]$ exactly. To account for this, we use the following relaxed notion of $(\alpha, \beta)$-\mcab.

\begin{definition}
    Let $\mC = \{c: \X \rgta \R\}$ be a collection of real-valued functions on $\X$, and $\D$ be a distribution $\X \times \zo$. We say that the partition $\mS$ of $\X$ is $(\alpha, \beta)$-\mcbd\ for $\mC, \D$ if there exists a distribution $\D'$ on $\X \times \zo$ such that $\dtv(\D, \D') \leq \beta$ and $\mS$ is $\alpha$-\mcbd\ for $\mC, \D'$. 
\end{definition}



==> comparison.tex <==

\section{Improved bounds for $\ell_1$ and $\ell_2$}

In this section, we proved better bounds for $\ell_1$ and $\ell_2$ loss. 


\subsection{$\ell_1$ loss and agnostic learning}





==> loss2.tex <==
\section{Differentiable loss functions}

The assumptions in the previous section do not apply for some commonly used loss functions including the exponential loss $\lexp(y, \hy) =\exp(-y\hy)$ and logistic loss,  given by $\llog(y, \hy) = \log(1 + \exp(-y\hy))$,
since for both these functions, the minima  occur as $\hy$ goes to $-\infty$.
We postulate properties that these (and other) loss functions have which suffice to prove that \mcab\ gives near optimal predictors. We require our loss functions to differentiable as a function of $\hy$, and we use $\ell'(y, \hy)$ to denote $\partial \ell/\partial \hy$. 

Consider the state $S_i$ where $\E_{\D_i}[\y] = \eta_i$. What constant value $t_i$ should we predict to minimize the loss? Let $\y \sim \eta_i$ denote a random variable $\y \in \pmo$ with expectation $\eta_i$. Define the expected loss function
    \begin{align}
    \label{ew:def-bar-l}
        \bar{\ell}(\eta_i, t)  = \E_{\y \sim \eta_i} [\ell(\y, t)] = \frac{1 + \eta_i}{2}\ell(1, t) +  \frac{1 - \eta_i}{2}\ell(-1, t).
    \end{align}
    and note that it is also convex and differentiable. Differentiating with respect to $t$, minima must satisfy the equation
    \begin{align}
    \label{eq:key}
        (1 + \eta_i)\ell'(1, t) +  (1 - \eta_i)\ell'(-1, t) = 0.
    \end{align}

The properties we need from our loss functions are that there exist minima where the derivative of $\ell$ is not too large. We state this formally below:


There exists $B >0$ so that for every $\eta_i \in (-1,1)$ there exists $t_i \in \R$ satisfying the following conditions:
\begin{enumerate}
    \item {\bf (Minimizes $\bar{\ell}$.)} $t_i$ is a minimum for $\bar{\ell}(\eta_i, t)$, hence it satsifies Equation \eqref{eq:key};
    \item {\bf (Boundedness.)} $|\ell'(1, t_i)(1 + \eta_i)| = |\ell'(-1, t_i)(1 - \eta_i)| \leq B$. 
\end{enumerate}
Note that the Equality in the boundedness condition is a consequence of Equation \eqref{eq:key},  


\begin{lemma}
\label{lem:lgt}
The logistic loss satisfies the condition above with $B =1/2$. 
\end{lemma}
\begin{proof}
    For the logistic loss
    \begin{align*}
        \llgt(y, t) = \log(1 + \exp(-yt))\\
        \llgt'(y, t) = \frac{-y\exp(-yt)}{1 + \exp(-yt)} = \frac{-y}{1 + \exp(yt)}
    \end{align*}
    Hence Equation \eqref{eq:key} can be rewritten as
    \begin{align*} 
        \frac{ 1 + \eta_i}{1 + \exp(t_i)} &= \frac{1 - \eta_i}{1 + \exp(-t_i)}\\
        \exp(t_i) &= \frac{1 + \eta_i}{1 - \eta_i}
    \end{align*}
    which has a unique solution for every $\eta_i \in (-1, 1)$. Moreover, this solution satisfies
    \begin{align*}
        |\ell'(1, t_i) (1 + \eta_i)| = \frac{1 + \eta_i}{1 + (1 + \eta_i)/(1 - \eta_i)} = \frac{1 - \eta_i^2}{2} \leq \fr{2}.
    \end{align*}   
\end{proof}

\begin{lemma}
\label{lem:exp}
The exponential loss satisfies the condition with $B =1$. 
\end{lemma}
\begin{proof}
    Since $\lexp(y,t) = \exp(- yt)$, we have 
    $\lexp'(y, t)= - y\exp(-yt)$.
    Hence Equation \eqref{eq:key} can be written as
    \begin{align*} 
        (1 + \eta_i)\exp(- t_i) &= (1 - \eta_i)\exp(t_i)\\
        \exp(2t_i) &= \frac{1 + \eta_i}{1 - \eta_i}
    \end{align*}
    which has a unique solution for $\eta_i \in (-1, 1)$. Further
    \begin{align*}
        |\ell'(1, t_i)|( 1+ \eta_i) &= \exp(-t_i)(1 + \eta_i) = \sqrt{\frac{1 - \eta_i}{1 + \eta_i}}(1 + \eta_i) = \sqrt{1 - \eta_i^2} \leq 1.
    \end{align*} 
\end{proof}
    Unlike for logistic loss, for exponential loss, $|\lexp'(1, t_i)|$ by itself might be unbounded, so the extra $(1 + \eta_i)$ factor in the boundedness condition is important.


\subsection{Multicalibration for differentiable losses}

Consider a \mcbd\ partition $\mS$, and a loss function $\ell$ satisfying these conditions. Consider the predictor $f_\mS$ such that $f_\mS(x) = t_i$ for all $x \in S_i$. We will show that restricted to each state $S_i$, $t_i$ is nearly a local minimum for the space of all small-norm linear functions in $\mC$.  Since $f_\mS$ is near-optimal for each state $S_i$ in the partition, it must be near-optimal overall. There are two steps to our proof:
\begin{enumerate}
    \item Show that \mcab\ implies that the gradient at $t_i$ is small (in $\ell_\infty$). 
    \item Show that the gradient condition implies that $t_i$ is near optimal for minimizing the expected loss over the space of all linear functions with small $\ell_1$ norm. 
\end{enumerate}



Let us consider a classifier of the form $g_w(x) = w_0 + \sum_{j \geq 1} w_jc_j(x)$ where $w = \{w_j\}$ is the vector of parameters. The loss $L(w)$ of this classifier is given by
\begin{align*}
    L(w) &= \E_{(\x, \y) \sim \D_i} \left[ \ell(\y g_w(\x))\right]
\end{align*}
Let $w^* = (t_i, \bf{0})$ denote the vector where $w_0 = t_i$ and $w_j = 0$ for all $j \geq 1$, so that $g_{w^*}(x) = t_i$.

\begin{lemma}
\label{lem:grad}
    Let $\grad L(w)$ denote the gradient of the loss function at $w$. Then we have
    \begin{align*}
        \fp{L}{w_0}(w^*)  & = 0\\
     \forall j\geq 1, \    \abs{\fp{L}{w_j}(w^*)} & \leq \alpha B
    \end{align*}
\end{lemma}
\begin{proof}
We first verify the claim for $w_0$. Differentiating wrt $w_0$ and plugging in $w_0 = t_i$ gives 
\[    \fp{L}{w_0}(w^*) = \frac{1 + \eta_i}{2}\ell(1, t_i) + \frac{1 - \eta_i}{2}\ell(-1, t_i) = 0.\] 
Differentiating with respect to $w_j$ for $j \geq 1$, we get 
\begin{align*}
    \fp{L}{w_j} &= \E_{(\x, \y) \sim \D} \left[ \ell'(\y, g_w(\x)) c_j(\x) \right]
\end{align*}
Plugging in $w = w^*$ so that $g_{w^*}(x) = t_i$, we get
\begin{align*}
    \fp{L}{w_j}(w^*)  &= \E_{(\x, \y) \sim \D} \left[ \ell'(\y, t_i) c_j(\x) \right] \\
    &= \E_{(\x, \y) \sim \D} \left[ \ell'(1, t_i) c_j(\x)\frac{1 + \y}{2} + \ell'(-1, t_i) c_j(\x)\frac{1 - \y}{2} \right] \\
    &= \frac{\ell'(1, t_i)}{2} \E_{(\x, \y) \sim \D} \left[ c_j(\x)(1 + \y) + \frac{\ell(-1, t_i)}{\ell'(1, t_i)}c_j(\x)(1 - \y) \right] \\
    &= \frac{\ell'(1, t_i)}{2} \E_{(\x, \y) \sim \D} \left[ c_j(\x)(1 + \y) - \frac{1 + \eta_i}{1 - \eta_i} c_j(\x)(1 - \y) \right] \\   
    &= \frac{\ell'(1, t_i)}{2(1 - \eta_i)} \E_{(\x, \y) \sim \D} \left[c_j(\x)(1 + \y)(1 - \eta_i) - c_j(\x)(1 - \y)(1 + \eta_i) \right] \\
    &= \frac{\ell'(1, t_i)}{1 - \eta_i}\E_{(\x, \y) \sim \D}[c_j(\x)(\y - \eta_i)]
\end{align*}
Hence by \mcab\ and the Boundedness condition,
\begin{align*}
   \left\lvert \fp{L}{w_j}(w^*)\right\rvert \leq \frac{|\ell'(t_i)| \alpha(1 - \eta_i^2)}{1 - \eta_i} = |\ell'(t_i)|(1 +\eta_i)\alpha \leq B \alpha
    \end{align*}
\end{proof}


Recall that $f^\ell_\mS: \X \rgta \R$ is the classifier where $f^\ell_\mS(x) =t_i$ for all $x \in S_i$, and that  $g_w(x) = w_0 + \sum_{j \geq 1} w_jc_j(x)$ is a linear classifier.  The next lemma is a simple consequence of convexity.
\begin{lemma}
\label{lem:convex}
For classifiers $f^\ell_\mS$ and $g_w$ as above, we have
    \[ \E_{\D}[\ell(\y, f^\ell_\mS(\x))] \leq  \E_{\D}[\ell(\y, g_w(\x))]+ \alpha B \|w\|_1. \] 
\end{lemma}
\begin{proof}
    We will prove that for every $i \in [m]$,
    \[ \E_{\D_i}[\ell(\y, t_i)] \leq  \E_{\D_i}[\ell(\y, g_w(\x))]+ \alpha B \|w\|_1. \]
    The claim then follows by averaging over the states. 
    
    We use the following property of (differentiable) convex functions $c: \X \rgta \R$: for all $y, x$, 
    \[ c(y) \geq c(x) + (y -x ) \cdot \nabla c (x).\]
    We now take $c = L$, $y = w$ and $x = w^*$ so that
    \[ L(w) \geq L(w^*) + (w - w^* ) \cdot \nabla L (w^*).\]
    We bound $|(w - w^* ) \cdot \nabla L (w^*)|$ using Holder's inequality. Firstly, the $0$ co-ordinate of the gradient is $0$ since
    \[ \fp{L}{w_0}(w^*) = 0 \]
    hence it does not contribute to the inner product. For $j \geq 1$, since $w^*_j =0$ we have 
    \[ \sum_{j \geq 1}|w_j - w_j^*|  = \sum_{j \geq 1}|w_j| = \|w\|_1. \]
    Whereas $\|\nabla L (w^*)\|_\infty \leq \alpha B$. So by Holder' inequality
    \[ |(w - w^* ) \cdot \nabla L (w^*)| \leq \alpha B \|w\|_1\]
    which implies that
    \[ L(w^*) \leq  L(w) + \alpha B \|w\|_1. \] 
    To complete the proof, we observe that 
    \begin{align*}    
        L(w^*) = \E_{\D_i}[\ell(\y, t_i)], \ \ L(w) = \E_{\D_i}[\ell(\y, g_w(\x))]. 
    \end{align*} 
\end{proof}




==> main.tex <==
\section{Introduction}

We show that a multicalibrated predictor with respect to the class $\mC$ achieves smaller classification error than each of the concepts in the class $\mC$.

\begin{theorem}
Consider a binary classification task with some joint distribution $\mu$ over the pair $(x,y)$ of datapoint $x\in \mX$ and label $y\in \{0,1\}$. Let $f: \mX\rightarrow[0,1]$ be any $\alpha$-multicalibrated predictor with respect to $\mC$, and let $\bar{f}: \mX\rightarrow \{0,1\}$ be the thresholded version of the predictor $f$, i.e. $\bar{f}(x)=\mathbf{1}(f(x)>0.5)$. Then,
\begin{align}
    \Pr_{(x,y)\sim \mu}[\bar{f}(x)\ne y] \le \min _{c\in\mC}\Pr_{(x,y)\sim \mu}[c(x)\ne y] + \alpha.
\end{align}
\end{theorem}
\begin{proof}
We first consider the special case when $\alpha=0$  since it is easiest to see the intuition there. Let $c^*=\argmin _{c\in\mC}\Pr_{(x,y)\sim \mu}[c(x)\ne y]$. Consider any set $S$ in the partition given by the multicalibrated predictor $f$. We claim that if the  predictions of $\bar{f}$ and $c^*$ differ in the set $S$, then $\bar{f}$ must be at least as good as $c^*$ in expectation over the datapoints in the set $S$. Let $C_1^*=\{x:c^*(x)=1\}$ and $C_0^*=\{x:c^*(x)=0\}$. Let $f(x)=p_S$ for $x\in S$. 
We first consider the case when $p_S>0.5$. In this case, $\bar{f}$ assigns the label 1 to all datapoints in $S$, and disagrees with $c^*$ on $T=C_0^*\cap S$. However, by the multicalibration property,
\begin{align*}
    \E_{(x,y)\sim \mu|x\in T}[y]=p_S>0.5.
\end{align*}
Therefore $\bar{f}$ must achieve strictly better prediction error than $c^*$ on $T$. Since they have the same prediction on the set $S-T$, $\tilde{f}$ must achieve strictly better prediction error than $c^*$ on the overall set $S$. An analogous argument shows that $\bar{f}$ is strictly better than $c^*$ when $p_S<0.5$, and is as good as $c^*$ when $p_S=0.5$. Therefore, $\bar{f}$ achieves overall prediction error at least as good as $c^*$.

We now consider the general case when $\alpha \ne 0$. Following the same argument as above, consider a set $S$ where the predictions of $\bar{f}$ and $c^*$ differ, and let $f(x)=p_S>0.5$ for $x\in S$. Let $T=C_0^*\cap S$ be defined as above. Note that by $\alpha$-multicalibration,
\begin{align*}
    p_S-\alpha \le \E_{(x,y)\sim \mu|x\in T}[y].
\end{align*}
This implies,
\begin{align*}
     \Pr_{(x,y)\sim \mu|x\in T}[\bar{f}(x)\ne y]&\le 1-p_S+\alpha\\
    \Pr_{(x,y)\sim \mu|x\in T}[c^*(x)\ne y]&\ge  p_S-\alpha.
\end{align*}
Therefore,
\begin{align*}
     \Pr_{(x,y)\sim \mu|x\in T}[\bar{f}(x)\ne y]-\Pr_{(x,y)\sim \mu|x\in T}[c^*(x)\ne y]&\le 1-2p_S+\alpha\le \alpha.
\end{align*}
Since $\bar{f}$ and $c^*$ have the same prediction on the set $S-T$, 
\begin{align*}
     \Pr_{(x,y)\sim \mu|x\in S}[\bar{f}(x)\ne y]-\Pr_{(x,y)\sim \mu|x\in S}[c^*(x)\ne y]\le \alpha.
\end{align*}
By an analogous argument, we can also show the above claim for the case when $p_S\le 0.5$. Therefore by taking the expectation over all sets $S$ in the partition,
\begin{align*}
     \Pr_{(x,y)\sim \mu}[\bar{f}(x)\ne y]-\Pr_{(x,y)\sim \mu}[c^*(x)\ne y]\le \alpha.
\end{align*}

\end{proof}

We show a simple example of a $p$-biased distribution where multicalibration with respect to the individual coordinates yields much smaller prediction error than any of the individual coordinates.

\begin{proposition}
Consider the distribution $P$ over $(x,y)$ where the distribution of the datapoint $x$ is uniform on the domain $\mX=\{0,1\}^n$ and the label $y$ is 0 for all $x$. Similarly, consider the distribution $Q$ over $(x,y)$ where the distribution of the datapoints $x$ is a $p$-biased distribution on the domain $\mX$ for some $p<1/3$ and the label $y$ is 1 for all $x$. Let $\mu=(P+Q)/2$. Let $\mC=\{x_i,i\in [n]\}$ be the hypothesis class which has the indicator functions on all the coordinates and let $f$ be any $\alpha$-multicalibrated predictor with respect to $\mC$. Then for some constant $\gamma>0$,
\begin{align}
    \Pr_{(x,y)\sim \mu}[f(x)\ne y]\le e^{-\gamma n}  < \min _{c\in\mC}\Pr_{(x,y)\sim \mu}[c(x)\ne y]=p/2.
\end{align}
\end{proposition}
\begin{proof}
(can add this if we plan on keeping this result)
\end{proof}

We show that multicalibration with respect to the individual coordinates lets us learn halfspaces with random noise, for any underlying distribution over the datapoints. 

\begin{theorem}
Consider a binary classification task over the domain $\mX=\{0,1\}^n$ with some distribution $D$ over the datapoints $x\in \mX$. Let $w$ be a vector in $\R^n$ such that each coordinate $w_i$ of $w$ is an integer, and let $h(x):\R^n\rightarrow\{\pm 1\}$ be the halfspace $h(x) = \sign(w^Tx)$. Let the label $y$ of any datapoint $x_i$ be $y=h(x)\cdot\eta(x)$, where $\eta(x)\in \{\pm1\}$ is a random variable independent of $x$ which is 1 with probability $(1-\eps)$ and $-1$ with probability $\eps$, for some $\eps\le 0.5$.  Let the concept class $\mC=\{x_i,i\in [n]\}$ consist of the indicator functions on all the coordinates. Then, for any predictor $f$ which $\alpha$-multicalibrated  with respect to $\mC$ for $\alpha=\gamma/\onenorm{w}$,
\begin{align}
    \Pr_{(x,y)\sim \mu}[f(x)\ne y]\le \eps + \gamma/2. 
\end{align}
\end{theorem}
\begin{proof}
We will show that if $h(x)$ is not constant on each set of the partition corresponding to the $\alpha$-multicalibrated predictor, then the partition cannot be $\alpha$-multicalibrated. Consider any set $S$ of the partition. Let $\E_{(x,y)\sim D|_S}[y]=\bar{y}_S$. Henceforth, all our expectations and probabilities will be with respect to the distribution $(x,y)\sim D|_S$ and hence we drop the subscript for brevity. We can write,
\begin{align*}
    \E[(y-\bar{y}_S)w^Tx] &= \E[yw^Tx]- \bar{y}_S)\E[w^Tx]\\
    &= \E[h(x)w^Tx\cdot \eta(x)] - \bar{y}_S\E[w^Tx]\\
    &= \E[\eta(x)]\cdot \E[\sign(w^Tx)w^Tx] - \bar{y}_S\E[w^Tx]\\
    &= (1-2\eps) \E[|w^Tx|]- \bar{y}_S\E[w^Tx].
\end{align*}
Note that since the noise $\eta(x)$ is independent of the datapoint $x$, $\bar{y}_S=\E[h(x)\cdot \eta(x)]={(1-2\eps)\E[h(x)]}$. Therefore we can simplify the above expression as follows,
\begin{align*}
    \E[(y-\bar{y}_S)w^Tx] &= (1-2\eps) \E[|w^Tx|]-(1-2\eps)\E[h(x)]\E[w^Tx]\\
    &\ge (1-2\eps)\E[|w^Tx|](1-|\E[h(x)]|).
\end{align*}
Note that $|w^Tx| \ge 1\; \forall \;x$ since each coordinate of $w_i$ is an integer, $x\in \{\pm 1\}^n$ and $w^Tx\ne 0$. Therefore,
\begin{align}
    \E[(y-\bar{y}_S)w^Tx] 
    &\ge (1-2\eps)(1-\E[h(x)]).\label{eq:discriminator}
\end{align}

Now, we rewrite the left hand side of the above equation as follows,
\begin{align*}
    \E[(y-\bar{y}_S)w^Tx]  &= \E[y(\sum_i w_ix_i)]-\bar{y}_S\sum_i  \E[w_ix_i]\\
    &= \sum_i w_i\E[yx_i]-\bar{y}_S\sum_i  w_i\E[x_i]\\
    &=\sum_i w_i \E[y|x_i=1]\Pr[x_i=1]
    - \bar{y}_S\sum_i  w_i \Pr[x_i=1]\\
    &= \sum_i w_i ( \Pr[x_i=1] (\E[y|x_i=1]-\bar{y}_S) \\
    &\le \sum_i |w_i| \max_i | \Pr[x_i=1] (\E[y|x_i=1]-\bar{y}_S) |\\
 %   &\le \sum_i |w_i| \max_i ( \max\{ |\E[y|x_i=1]-\bar{y}_S|,|\E[y|x_i=-1]-\bar{y}_S|\})\\
    &= \onenorm{w} \max_i  |\E[y|x_i=1]-\bar{y}_S|.
\end{align*}
Therefore by \eqref{eq:discriminator},
\begin{align*}
   \max_i  |\E[y|x_i=1]-\bar{y}_S| \ge \frac{(1-2\eps)(1-|\E[h(x)]|)}{\onenorm{w}}.
\end{align*}
Now, if $f$ is $\alpha$-multi-calibrated for $\alpha=\gamma/\onenorm{w}$ then,
\begin{align}
    \frac{(1-2\eps)(1-|\E[h(x)]|)}{\onenorm{w}} &\le \frac{\gamma}{\onenorm{w}},\nonumber\\
    \implies |\E[h(x)]| &\ge 1-\frac{\gamma}{1-2\eps}.\label{eq:bias1}
\end{align}
Note that the prediction $b_S$ of the multicalibrated predictor $f$ on the set $S$ is $b_S=\sign(\bar{y}_S)={\sign((1-2\eps)\E[h(x)])}=\sign(\E[h(x)]$, since $\eps\le 0.5$. Note that,
\begin{align}
    \Pr[h(x)=b]=\frac{1+|\E[h(x)]}{2}
    &\ge 1-\frac{\gamma}{2(1-2\eps)}\label{eq:bias2}
\end{align}
where we use \eqref{eq:bias1} to get the lower bound. The error of $\bar{f}$ on the set $S$ is,
\begin{align*}
    \Pr[\bar{f}\ne y] &= \eps \Pr[h(x)=b] + (1-\eps) (1- \Pr[h(x)=b])\\
    &= 1-\eps -\Pr[h(x)=b](1-2\eps).
\end{align*}
Since $\eps\le 0.5$, we can use \eqref{eq:bias2} to obtain,
\begin{align*}
    \Pr[\bar{f}\ne y] &\le 1-\eps -(1-\frac{\gamma}{2(1-2\eps)})(1-2\eps)\\
    &\le \eps + \gamma/2.
\end{align*}
Since the above is true for any set $S$ in the partition, the result follows.

\eat{

To begin, we first consider the case where $\E_{x\sim D|_S}[g(x)]=0$. 
\begin{lemma}\label{lem:balanced}
For any set $S$ in the partition, consider some distribution $P$ over $x\in S$ such that $\E_{x\sim P}[g(x)]=0$. Let $\alpha_0=\frac{\eps}{\onenorm{w}}$. Then there exists some coordinate $x_i$ such that either,
\begin{align*}
    \min\{|\E_{x\sim P|_{x_i=1}}[y]|,| \E_{x\sim P|_{x_i=-1}}[y]|\} > \alpha_0.
\end{align*}
This implies that the set $S$ is not $\alpha_0$-calibrated for at least one of $S\cap x_i=1$ and $S\cap x_i=0$. 
\end{lemma}
\begin{proof}
We will use the following discriminator lemma which intuitively says that any halfspace must be correlated with one of the coordinates.
\begin{lemma}\label{lem:discriminator}
Consider any halfspace $g(x) = \sign(w^Tx)$ where every coordinate $w_i$ of $w$ is an integer. Then for any probability distribution $D$ over $x\in \mX$, there must be some $x_i$ such that, $$\left|\E_{x\sim D} [g(x)x_i]\right|\ge \frac{1}{\onenorm{w}}.$$
\end{lemma}
\begin{proof}
Note that $|w^Tx| \ge 1$ since each coordinate of $w_i$ is an integer, $x\in \{\pm 1\}^n$ and $w^Tx\ne 0$. Therefore,
\begin{align*}
    \E[g(x)w^Tx] = \E[\sign(w^Tx)w^Tx]= \E[|w^Tx|] \ge 1.
\end{align*}
We can rewrite the above as follows,
\begin{align*}
    \E[g(x) w^T x] = \E[g(x)(\sum_i w_i x_i)] = \sum_i w_i \E[g(x) x_i] \ge 1.
\end{align*}
Therefore,
\begin{align*}
    \sum_i |w_i|\max_i|\E[g(x) x_i]| &\ge 1\\
    \implies \max_i|\E[g(x) x_i]| &\ge \frac{1}{\onenorm{w}}.
\end{align*}
\end{proof}
Since the noise $\eta_i$ is independent, \begin{align*}
    \E_{x\sim P} [yx_i] = \E_{x\sim P} [g(x)x_i\cdot \eta_i]=\E_{x\sim P} [g(x)x_i]\cdot \E[\eta_i] =\eps\E_{x\sim P} [g(x)x_i].
\end{align*}
It then follows using Lemma \ref{lem:discriminator} that there exists some coordinate $x_i$ such that, 
\begin{align}
    \left|\E_{x\sim P} [yx_i]\right| \ge \frac{\eps}{\onenorm{w}}.\label{eq:distinguish}
\end{align}
We claim that this implies that the set is not $\alpha_0$-calibrated with respect to $x_i$, for $\alpha_0=\frac{\eps}{\onenorm{w}}$. Let $p_1=\E_{x\sim P|_{x_i=1}}[y]$ and $p_2=\E_{x\sim P|_{x_i=-1}}[y]$. Note that,
\begin{align*}
    \E_{x\sim P} [yx_i]=p_1\cdot \Pr_{x\sim P}[x_i=1] -p_2\cdot \Pr_{x\sim P}[x_i=-1].
\end{align*}
Therefore, by \eqref{eq:distinguish}, $\min\{p_1,p_2\}\ge \alpha_0$. If $\alpha<\alpha_0$, this implies that the $\alpha_0$-calibration condition is not satisfied for at least one of $S\cap x_i=1$ and $S\cap x_i=0$.
\end{proof}

We now consider the case when $\E_{x\sim D|_S}[g(x)]=\beta$. Our argument works by reweighing the distribution $D|_S$ to reduce to the case when $\E_{x\sim D|_S}[g(x)]=0$ and then using the Lemma \ref{lem:balanced}.

For all $x\in S$ and some constants $\gamma_1$ and $\gamma_2$, define a new distribution $D'|_S$ by reweighing $x$ such that $g(x)=1$ by $\gamma_1$ and $x$ such that $g(x)=-1$ by $\gamma_2$. We choose $\gamma_1=1/(1+\beta)$ and $\gamma_2=1/(1-\beta)$ which ensures,
\begin{gather*}
    \Pr_{x\sim D'|_S}[x:g(x)=1] = \Pr_{x\sim D'|_S}[x:g(x)=-1] = 1/2,\\
    \implies \E_{x\sim D'|_S}[g(x)]=0.
\end{gather*}
}

\end{proof}

We show that halfspaces are not agnostically learnable with the individual coordinates being the weak learners.

\begin{proposition}
Consider a binary classification task with some distribution $D$ over the datapoints $(x,y)$ where $x \in \{0,1\}^{n}$ and $y \in\{\pm 1\}$. Let the concept class $\mC=\{x_i,i\in [n]\}$ consist of the indicator functions on all the coordinates. Then there exists a distribution $D$ such that the class of halfspaces $h(x) = \sign(w^Tx)$ is not agnostically learnable using a weak learner for the class $\mC$.
\end{proposition}
\begin{proof}
Consider the distribution on $(x, y)$ where $y = x_1 \oplus x_2 \oplus x_3$ is the parity function on the first three variables. Then the labels are uncorrelated with any $x_i$. However the majority of $(x_1, x_2, x_3)$ is correct with probability $3/4$.
\end{proof}


%Let be supported on the subset of the domain where $x_1=1$, and is uniform over this support. We use the parity function as a counterexample. Let $q(x)=\sum_i x_i \mod 2$. Consider $h(x) = \text{majority} (x_2,\dots, x_n)=\sign(\sum_{i=2}^n x_i-(n-1)/2)$. 


We show that a multicalibrated predictor with respect to the class $\mC$ achieves smaller regression error than any sparse linear combination of the concepts in the class $\mC$.

\begin{theorem}
Consider a binary classification task with some distribution $D$ over the datapoints in the domain $\mX$. Let $p^*(x)$ be the conditional distribution of the label $y$ for any $x$. Consider some concept class $\mC$ with cardinality $|\mC|$ with concepts $\{c_i(x):i \in [|\mC|]\}$ where $c_i(x) : \mX\rightarrow \{0,1\}$. Let ${\mG}$ be the class of functions ${\mG}=\{\sum_i w_i c_i(x): w_i \in \R^{|\mC|}, \onenorm{w}=W\}$. Let $f$ be any $\alpha$-multicalibrated predictor with respect to $\mC$. Then for any $g\in \mG$,
\begin{align}
    \E\norm{g(x)-p^*(x)}^2 &\ge \E\norm{ f(x)-p^*(x)}^2+ \E\norm{g(x)- f(x)}^2 -2\alpha\onenorm{w}.
\end{align}
\end{theorem}
\begin{proof}
Consider any set $S$ of the partition. Let $\E_{(x,y)\sim D|_S}[p^*(x)]=\bar{y}_S$. Henceforth, all our expectations and probabilities will be with respect to the distribution $(x,y)\sim D|_S$ and hence we drop the subscript for brevity. Note that $f(x) = \bar{y}_S$ for $x\in S$. For any predictor $g(x)$, we can write,
\begin{align}
    \E\norm{g(x)-p^*(x)}^2 &=\E\norm{(g(x)- \bar{y}_S) - ( p^*(x)-\bar{y}_S)}^2\nonumber\\
    &= \E\norm{g(x)- \bar{y}_S}^2 + \E\norm{ p^*(x)-\bar{y}_S}^2 +2\E[(g(x)- \bar{y}_S)(p^*(x)-\bar{y}_S)]\nonumber\\
    &= \E\norm{g(x)- \bar{y}_S}^2 + \E\norm{ p^*(x)-\bar{y}_S}^2 +2\E[g(x)(p^*(x)-\bar{y}_S)]\label{eq:regression}
\end{align}
where the last step follows since $\E[p^*(x)]=\bar{y}_S$. Since $g(x) = \sum_i w_i c_i(x)$,
\begin{align*}
    \E[g(x)(p^*(x)-\bar{y}_S)] &= \sum_i w_i \E[c_i(x)(p^*(x)-\bar{y}_S)]\\
    &= \sum_i w_i (\E[c_i(x)p^*(x)]-\bar{y}_S\E[c_i(x)])\\
    &= \sum_i w_i (\E[p^*(x)|c_i(x)=1]\Pr[c_i(x)=1]-\bar{y}_S\Pr[c_i(x)=1])\\
    &= \sum_i w_i \Pr[c_i(x)=1] (\E[p^*(x)|c_i(x)=1]-\bar{y}_S).
\end{align*}
Therefore, 
\begin{align*}
   | \E[g(x)(p^*(x)-\bar{y}_S)]| &\le \sum_i |w_i|  |\E[p^*(x)|c_i(x)=1]-\bar{y}_S|\\
   &\le  \sum_i |w_i| \max_i |\E[p^*(x)|c_i(x)=1]-\bar{y}_S|\\
   &= \onenorm{w}\max_i |\E[p^*(x)|c_i(x)=1]-\bar{y}_S|.
\end{align*}
Note that if $f$ is $\alpha$-multi-calibrated, then
\begin{align*}
    \max_i |\E[p^*(x)|c_i(x)=1]-\bar{y}_S| \le \alpha. 
\end{align*}
Therefore if $f$ is $\alpha$-multi-calibrated,
\begin{align*}
   | \E[g(x)(p^*(x)-\bar{y}_S)]| &\le \alpha\onenorm{w}.
\end{align*}
Plugging this into \eqref{eq:regression},
\begin{align*}
    \E\norm{g(x)-p^*(x)}^2 &\ge \E\norm{g(x)- \bar{y}_S}^2 + \E\norm{ p^*(x)-\bar{y}_S}^2 -2\alpha\onenorm{w}.
\end{align*}
Since this is true for any $S$, averaging over all sets $S$ in the partition gives the desired result.
\end{proof}

\begin{theorem}
Consider a regression task with some distribution $D$ over the datapoints in the domain $\mX$. Let the conditional distribution $p^*(x)$ of the label $y$ for any $x$ be $u(\sum_{i=1}^n w_i x_i)$, for some monotonic and $L$-Lipchitz function $u$. Let the concept class $\mC$ be the set of all thresholds on the individual coordinates, i.e.  $\mC=\{I(x_i \diamond \theta):i \in [n], \theta\in \R, \diamond \in \{>,<,\ge, \le \}\}$.  Let $f$ be any $\alpha$-multicalibrated predictor with respect to $\mC$. Then,
\begin{align}
    \E\norm{f(x)-p^*(x)}^2 \le  \alpha L\onenorm{w}.
\end{align}
\end{theorem}
\begin{proof}
Consider any set $S$ in the partition corresponding to the multicalibrated predictor $f$. Define $\sigma_{p^*|S}^2=\E_{|S}[(p^*(x)-\E_{|S}[p^*(x)])^2]$ as the variance of $p^*$ in the set $S$. Henceforth, all our expectations and probabilities will be with respect to the distribution $(x,y)\sim D|_S$ and hence we drop the subscript for brevity. By Lemma 4 of [Adam's awesome paper], there exists an $i\in [n] , \theta\in \R,$ and $\diamond \in \{>,<,\ge, \le \}$ such that,
\begin{align*}
    \E[p^*(x)|I(x_i \diamond \theta)]\Pr[x_i \diamond \theta]-\E[p^*(x)]\Pr[x_i \diamond \theta]\ge \frac{\sigma_{p^*|S}^2}{L\onenorm{w}}.
\end{align*}
But by $\alpha$-multicalibration,
\begin{gather*}
 |\E[p^*(x)|I(x_i \diamond \theta)]-\E[p^*(x)]|\le \alpha,  \\  \implies |\E[p^*(x)|I(x_i \diamond \theta)]\Pr[x_i \diamond \theta]-\E[p^*(x)]\Pr[x_i \diamond \theta]|\le \alpha.
\end{gather*}
Therefore, $\alpha$-multicalibration implies that, 
\begin{align*}
    \frac{\sigma_{p^*|S}^2}{L\onenorm{w}} \le \alpha.
\end{align*}
Note that $f(x)=\E_{|S}[p^*(x)]$ for all $x\in S$. Therefore, for all $x\in S$,
\begin{align*}
    \E[(f(x)-p^*(x))^2]\le \alpha L\onenorm{w}.
\end{align*}
Since this is true for every set $S$, by averaging over all sets $S$ we get the final result. 
 
\end{proof}

\section{Simplifying and characterizing agnostic boosting}

In this section we characterize agnostic boosting -- it is equivalent to just learning linear combinations of weak learners!? The intuition is that one can define an inner product $cor(h, f) =E[h(x)f(x)]$ and argue that if class $H$ is weak-agnostic-learned by $C$ then $H$ is close to $span(C)$.

Let $Y=\{-1,1\}$ and let $H, C \subseteq Y^X$ be families of binary classifiers. Let $D$ be a distribution over a finite or countably infinite\footnote{Measure theory sucks.} set $X$. The target function to be learned is $f: X \rightarrow [-1,1]$. It is sometimes assumed that $f: X \rightarrow Y$ is binary, and moreover for  (realizable) PAC it is further assumed that $f \in H$. But for general agnostic learning $f: X \rightarrow [-1,1]$ can be interpreted as: an example $x \sim D$ is drawn and the label $y \in Y$ is chosen so that $\E[y|x] = f(x)$. Define correlation $cor_D(h, f) = E_{x \sim D}[h(x)f(x)]$. This is just $1-2Pr[h(x)\neq y]$ so $cor>0$ means error is less than 1/2, and correlation 1 means error is 0. 

Let $L$ be a learning algorithm that outputs binary classifiers in $C$. 
As background, in standard (noiseless)boosting one says that $L$ $\gamma$-weak-learns $H$ if for every classifier $f \in H$ and every distribution $D$ over $X$, with probability $\geq 3/4$, $L$ outputs $c \in C$ with correlation $cor_D(c, f)\geq \gamma$. It is known that $H \subseteq maj(C)$ the majority of sums of classifiers in $C$. Moreover the algorithm that finds $c \in C$ with maximum correlation (if it could be done efficiently) would $\gamma$ weak-learn the class $H=maj_k(C)$ of the majority of the sum of up to $k$ classifiers in $C$ with $\gamma = \poly(1/k)$. 

In agnostic learning, we consider a target function $f:X \rightarrow [-1,1]$. Again suppose we have an algorithm $L$ that outputs binary classifiers in $C$. One says that $L$ $(\gamma, \alpha, D)$-weak-agnostic learns $C$ if for every classifier $f:X \rightarrow [-1,1]$ with $\max_{h \in H} cor_D(h, f) \geq \alpha$, with probability $\geq 3/4$ $L$ outputs $c \in C$ with $cor_D(c, f) \geq \gamma$. This is stronger than standard boosting in that it has to work for any $f$ that has $\geq \alpha$ correlation with some $h \in H$, as opposed to standard learning where it only has to work for those $f$ where OPT$=0$) and moreover it only has to hold for some $D$. It is known that $L$ efficiently $(\gamma, \alpha, D)$-weak-agnostic learns $H$ then one can efficiently find a classifier with correlation $> OPT-\alpha - \eps$  (OPT$=max_{h \in H} cor(h, f)$), with high probability, in time $\poly(1/\eps, 1/\gamma, 1/\alpha)$.

Ideally, for agnostic boosting to show that one can agnostically learn $H$, one would like $L$ that agnostically $(\gamma(\alpha), \alpha, D)$-weak learns $H$ where $\gamma : (0,1] \rightarrow (0,1]$, so we can achieve correlation $>OPT - 2\epsilon$ by setting $\alpha =\epsilon$. In the TODOs, we ask whether a version of this might be provable for specific $(\gamma, \alpha)$ pairs.

\begin{proposition}
Fix distribution $D$ with full support\footnote{This full-support assumption can probably be removed with care} over $X$, and $H, C \subseteq Y^X$. Suppose there is some function $\gamma : (0,1] \rightarrow (0,1]$ such that for all $f: X \rightarrow [-1,1]$,
$$\sup_{c \in C} cor_D(c, f) \geq \gamma(\sup_H cor(h, f)).$$
Then $H \subseteq span(C)$.
\end{proposition}
\begin{proof}
Suppose not. Then there is some $h \in H$ such that $h \not\in span(C)$. Take $h' \in span(C)$ that is closest in L2 norm to $h$, i.e., that minimizes squared error $E_D[(h(x)-h'(x))^2]$. TODO: argue that $cor(h', h)<1$ otherwise a scaled-down version of $h'$ would have lower squared error.

Now,  take $f=\frac{h-h'}{Z}$ where $Z$ is a normalization constant large enough to guarantee that $f(x)\in [-1,1]$. Clearly no $c \in C$ has positive correlation with $f$ and yet there $$cor(h, f) = \frac{1}{Z}(cor(h, h)-cor(h', h)) \frac{1}{Z}(1-cor(h', h)) > 0.$$ 
\end{proof}

\subsection{TODOs: would be nice to do}
\begin{enumerate}
    \item Check that this is right? 
    \item Add analysis for approximate case, i.e., some version of the above that only holds for specific ($\gamma, \alpha$) where it would have to be shown that everything in $H$ is close to the span of $C$ (with bounded weights) or something like that.
    \item Show that gradient boosting or some very simple boosting algorithm works in this setting?
\end{enumerate}



==> optimaler.tex <==

Is this interesting enough to include/prove???
